Classification and Construction of Topological Phases of Quantum Matter

We develop a theoretical framework for the classification and construction of symmetry protected topological (SPT) phases, which are a special class of zero-temperature phases of strongly interacting gapped quantum many-body systems that exhibit topological properties. The framework unifies various proposals for the classification of SPT phases, including the group (super-)cohomology proposal, the (spin-)cobordism proposal, the Freed-Hopkins proposal, and the Kitaev proposal. The power of the framework is demonstrated in a number of applications: (1) the classification and construction of 3D fermionic SPT phases in Wigner-Dyson classes A and AII with glide symmetry, (2) the classification and construction of 3D bosonic SPT phases with space-group symmetries for all 230 space groups, (3) the derivation of a Mayer-Vietoris sequence relating the classification of SPT phases with and without reflection symmetry, and (4) an interpretation of the structure of general crystalline SPT phases via the Atiyah-Hirzebruch spectral sequence. The framework is based on Kitaev's idea that short-range entangled states form what are known as $\Omega$-spectra in the sense of algebraic topology, and models the classification of SPT phases by what are called generalized cohomology theories.

==> frontmatter/abstract.tex <==

% the abstract

We develop a theoretical framework for the classification and construction of symmetry protected topological (SPT) phases, which are a special class of zero-temperature phases of strongly interacting gapped quantum many-body systems that exhibit topological properties. The framework unifies various proposals for the classification of SPT phases, including the group (super-)cohomology proposal, the (spin-)cobordism proposal, the Freed-Hopkins proposal, and the Kitaev proposal. The power of the framework is demonstrated in a number of applications: (1) the classification and construction of 3D fermionic SPT phases in Wigner-Dyson classes A and AII with glide symmetry, (2) the classification and construction of 3D bosonic SPT phases with space-group symmetries for all 230 space groups, (3) the derivation of a Mayer-Vietoris sequence relating the classification of SPT phases with and without reflection symmetry, and (4) an interpretation of the structure of general crystalline SPT phases via the Atiyah-Hirzebruch spectral sequence. The framework is based on Kitaev's idea that short-range entangled states form what are known as $\Omega$-spectra in the sense of algebraic topology, and models the classification of SPT phases by what are called generalized cohomology theories.


==> frontmatter/previousworks.tex <==


Portions of the following previously published works by the author of this dissertation (``Charles Zhaoxi Xiong") appear in this dissertation:

\begin{itemize}
\item {\bf Minimalist approach to the classification of symmetry protected topological phases}

Charles Zhaoxi Xiong

Journal of Physics A: Mathematical and Theoretical, 51 (44):445001, 2018

DOI: 10.1088/1751-8121/aae0b1

URL: \href{http://stacks.iop.org/1751-8121/51/i=44/a=445001}{http://stacks.iop.org/1751-8121/51/i=44/a=445001}

\item {\bf Organizing symmetry-protected topological phases by layering and symmetry reduction: A minimalist perspective}

Charles Zhaoxi Xiong and A. Alexandradinata

Physical Review B, 97:115153, 2018

DOI: 10.1103/PhysRevB.97.115153

URL: \href{https://link.aps.org/doi/10.1103/PhysRevB.97.115153}{https://link.aps.org/doi/10.1103/PhysRevB.97.115153}

\item {\bf Generalized homology and Atiyah-Hirzebruch spectral sequence in crystalline symmetry protected topological phenomena}

Ken Shiozaki, Charles Zhaoxi Xiong, and Kiyonori Gomi

arXiv:1810.00801 [cond-mat.str-el], 2018

URL: \href{https://arxiv.org/abs/1810.00801}{https://arxiv.org/abs/1810.00801}

\item {\bf Bosonic Crystalline Symmetry Protected Topological Phases Beyond the Group Cohomology Proposal}

Hao Song, Charles Zhaoxi Xiong, and Sheng-Jie Huang

arXiv:1811.06558 [cond-mat.str-el], 2018

URL: \href{https://arxiv.org/abs/1811.06558}{https://arxiv.org/abs/1811.06558}
\end{itemize}




==> frontmatter/thanks.tex <==

% the acknowledgments section

I would like to begin by thanking my thesis advisor, Prof.\,Ashvin Vishwanath, and my committee members, Prof.\,Subir Sachdev and Prof.\,Aurther Jaffe. There are many people who have helped and supported me during my PhD, which I started at the University of California, Berkeley in 2014 and continued at Harvard University in 2016. I have learned much of the classical works in the field of topological phases from the special topics classes, Physics 216 by Prof.\,Ashvin Vishwanath and Physics 250 by Prof.\,Joel Moore, offered at UC Berkeley in Fall 2014. I have acquired the bulk of my knowledge in albegraic topology from Math 215B by Prof.\,Richard Bamler, also at UC Berkeley, in Spring 2015. I first began to understand generalized cohomology theories, which have become an integral part of my PhD research, through discussions with such mathematical physicists as Ryan Thorngren and Ammar Husain. Throughout the years I have had numerous helpful discussions with my colleagues Sho Sugiura, Yingfei Gu, Yi-Ting Hsu, Zhen Bi, Abhishodh Prakash, Shenghan Jiang, Chang-Tse Hsieh, Yi Zhang, Jong Yeon Lee, Dan Borgnia, Wen Wei Ho, and many others.

I would like to give special thanks to my collaborators: Aris Alexandradinata, Judith H\"oller, Dominic Williamson, Prof.\,Ken Shiozaki, Prof.\,Kiyonori Gomi, Hao Song, and Shengjie Huang. I learned a lot about noninteracting topological phases---topological insulators and superconductors---from Aris, who was my first collaborator during graduate school. Aris was very easy to work with, and has continued to be a dear friend. At this moment, he is a postdoctoral fellow at the University of Illinois, Urbana-Champaign and searching for faculty positions. I wish him the best of luck. Judith, whom I first met at the Boulder School for Condensed Matter and Materials Physics in 2016, has been a close and supportive friend. We share a lot of interest in the mathematical aspects of topological phases. She has been a source of encouragement at moments of intellectual isolation during graduate school. I wish her well going forward regardless of the path she chooses. Dominic, whom I met in a project with Judith, has endowed me with substantial knowledge in the topic of matrix product states. The latter has proven useful in my later project in machine learning, which is not included in this thesis. Ken, whom I met at the APS March Meeting in 2018, and his long-term collaborator, Kiyonori, whom I have not met in person, are both professors in Japan. They were great to work with, and they are great people who have treated me as a human being with respect. Hao Song, whom I recently met, and Shengjie Huang, whom I met at the 2016 Boulder School, have given me a bunch of inspirations relating to crystalline topological phases. They are both conscientious scientists, and I much appreciate their integrity.

I also received a great deal of help from Anne Takizawa, who was a staff member in the Physics Student Services at UC Berkeley, in my first two years in graduate school. I have worked with her on so many things, from fulfilling course requirements to preliminary exams to organizing poster session. She is someone who really puts herself in students' shoes. I just learned---and could not believe---that she retired in 2017, a year after I transferred to Harvard University. I wish I would see her as I return to the Bay Area. I am also grateful for the copious help I received from Jacob Barandes, who is now the Director of Graduate Studies for FAS Science and Co-director of Graduates Studies for Physics at Harvard, and Lisa Cacciabaudo, who is the Graduate Program Administrator at Harvard Physics, around the time I transferred to Harvard University and throughout the years that followed. They made me feel welcome as someone who joined the program midway. I would also like to give a shout-out to Elizabeth Alcock, who is the assistant to Prof.\,Vishwanath and therefore takes care of administrative work that involves us. She does an excellent job and I am very thankful for her help in the past few years.

A ``thank you" is not nearly enough for those who have been there for me when I was in despair, when I was in need, when I was struggling, and who have given me the greatest gifts in this insane journey called PhD. Ashvin, Aris, and Emma: thank you for helping me find my next step after the PhD. Alex: thank you for staying true to yourself. Judith: thank you for always being there for me; you have helped me in ways you do not understand. Sachi, Sandy, Michael, Shubhayu, Chris, Erik, and Stephen: thank you for all the fun you brought me over the years. Anisa: thank you for standing up for what you believe and what is right. Ioana: thank you for always being so open and genuine; I am grateful to know you. Can: thank you for your support in my most vulnerable times. Yasaman: you are an incredible human being and have always been a trusted friend; I look forward to seeing you a lot more. Finally, to my significant other, Tatiana: thank you, so much, for all your love and support; I would not be who I am without you.

\begin{center}
$\ast$\hspace{0.2in}$\ast$\hspace{0.2in}$\ast$
\end{center}

This thesis was typeset using \LaTeX, originally developed by Leslie Lamport and based on Donald Knuth's \TeX.
%The body text is set in 11 point Egenolff-Berner Garamond, a revival of Claude Garamont's humanist typeface.
%The above illustration, \textit{Science Experiment 02}, was created by Ben Schlitter and released under \href{http://creativecommons.org/licenses/by-nc-nd/3.0/}{\textsc{cc by-nc-nd 3.0}}.
A template that can be used to format a PhD dissertation with this look \textit{\&} feel has been released under the permissive \textsc{agpl} license, and can be found online at \href{https://github.com/suchow/Dissertate}{github.com/suchow/Dissertate} or from its lead author, Jordan Suchow, at \href{mailto:suchow@post.harvard.edu}{suchow@post.harvard.edu}.

